Shielded Reinforcement Learning for Hybrid Systems

Safe and optimal controller synthesis for switched-controlled hybrid systems, which combine differential equations and discrete changes of the system's state, is known to be intricately hard. Reinforcement learning has been leveraged to construct near-optimal controllers, but their behavior is not guaranteed to be safe, even when it is encouraged by reward engineering. One way of imposing safety to a learned controller is to use a shield, which is correct by design. However, obtaining a shield for non-linear and hybrid environments is itself intractable. In this paper, we propose the construction of a shield using the so-called barbaric method, where an approximate finite representation of an underlying partition-based two-player safety game is extracted via systematically picked samples of the true transition function. While hard safety guarantees are out of reach, we experimentally demonstrate strong statistical safety guarantees with a prototype implementation and UPPAAL STRATEGO. Furthermore, we study the impact of the synthesized shield when applied as either a pre-shield (applied before learning a controller) or a post-shield (only applied after learning a controller). We experimentally demonstrate superiority of the pre-shielding approach. We apply our technique on a range of case studies, including two industrial examples, and further study post-optimization of the post-shielding approach.

==> graphics/RWSynthesis.tex <==
\begin{tabular}{@{\hspace{3mm}} c @{\hspace{3mm}} c @{\hspace{3mm}} c } 
\toprule
\textbf{$\granularity~~$}	&	\textbf{Seconds}	&	\textbf{Probability safe}\\
\midrule
0.1	&	0	&	Considers $s_0$ unsafe	\\
\midrule
0.01	&	3	&	$\geq 91.4112$\% (1\% CI)	\\
\midrule
0.005	&	33	&	$\geq 91.4112$\% (1\% CI)	\\
\end{tabular}
